Meta-Analysis of Randomized Experiments with Applications to Heavy-Tailed Response Data

A central obstacle in the objective assessment of treatment effect (TE) estimators in randomized control trials (RCTs) is the lack of ground truth (or validation set) to test their performance. In this paper, we propose a novel cross-validation-like methodology to address this challenge. The key insight of our procedure is that the noisy (but unbiased) difference-of-means estimate can be used as a ground truth ``label" on a portion of the RCT, to test the performance of an estimator trained on the other portion. We combine this insight with an aggregation scheme, which borrows statistical strength across a large collection of RCTs, to present an end-to-end methodology for judging an estimator's ability to recover the underlying treatment effect as well as produce an optimal treatment "roll out" policy. We evaluate our methodology across 699 RCTs implemented in the Amazon supply chain. In this heavy-tailed setting, our methodology suggests that procedures that aggressively downweight or truncate large values, while introducing bias, lower the variance enough to ensure that the treatment effect is more accurately estimated.

==> aggregation.tex <==
%!TEX root = main.tex
\section{An Aggregation Scheme}
\label{app:agg}
As briefly touched upon in \cref{sec:val}, aggregating the mean-squared errors requires handling a practical consideration. Since the RCTs and interventions across RCTs themselves may be different, the overall scales of the MSEs between different RCTs may be different. As an example, consider a corpus of two RCTs on which estimator $A$ obtain errors $\{1, 10\}$ and estimator $B$ obtains errors $\{2 , 9\}$. Simply averaging the errors or doing a rank-based test of performance would indicate both estimators are equivalent. However, intuitively we believe a relative improvement of estimator $B$ from $10$ to $9$ on the second RCT does not outweigh the degradation from $1$ to $2$ on the first RCT.

This observation motivates the definition of a normalized score to compare the estimators $A$ vs $B$, as a function of the vectors of their noisy errors.\footnote{As noted earlier, in practice each error estimate is averaged over several resampled train/test splits, but we suppress this extra notation for clarity.} For each intervention $i \in \{I_1,...,I_N\}$ we define the normalized score (already introduced in \eqref{eq:normalize_obj})):
\begin{align}
	S_i(\hat{A}_i, \hat{B}_i) = \frac{\hat{B}_i-\hat{A}_i}{\hat{B}_i + \hat{A}_i}, %\label{eq:normalize_obj}
\end{align}
for $\hat{A}_i \in \hat{\A}$ and $\hat{B}_i \in \hat{\B}$. Where $\hat{\A}$ and $\hat{\B}$ are defined according to \cref{def:Aset} and \cref{def:Bset} respectively.

This normalized score vector (which we denote by $\score(\hat{\A}, \hat{\B})$) implicitly binarizes each of its elements to bound them in the range $[-1, 1]$. Each element of this vector is a noisy score of estimator $A$'s performance relative to $B$ \textit{on one RCT in the corpus}.\footnote{Our notion of a normalized score vector is element-wise transitive. That is, $\frac{b-a}{a+b} > 0$ and $\frac{c-b}{b+c} > 0$ imply $\frac{c-a}{a+c}>0$.} If the estimator has many elements that are positive, it suggests that estimator $B$ has larger errors than estimator $A$. In this case, we would expect estimator $A$ to be better than estimator $B$.

To formalize this intuition, we use the following heuristic which implicitly treats each RCT equally independent of size. We use a two-sided one-sample $t$-test applied to this normalized score vector to test the null that the ``population mean" of the $\score$ ``distribution" is $0$, i.e., that the performance of estimator $A$ is indistinguishable from the performance of estimator $B$. Overall, this procedure interpolates between two extremes. A purely rank-based test of performance might only count the number of RCTs for which $A$ is better than $B$ irrespective of how much better one is in a particular RCT. Meanwhile, a procedure which only looks at the raw (unnormalized) RCT errors has the property that RCTs with large MSE values for both estimators would drown out signal from RCTs with small MSE values. We stress that the $t$-test heuristic provides a simple way of converting the information contained in $\score(\hat{\A}, \hat{\B})$ to a single number, but we recommend looking at the score histograms for a more complete picture.

==> estimators.tex <==
%!TEX root = main.tex
\section{Estimators}
\label{app:estimators}
In this Appendix we formally define the estimators used in the paper.

For the following estimators, we note that each admits a ``Winsorization" which can be used to trade off bias and variance. To do this, we can simply Winsorize the covariates and targets, $X, D, Y$, \textit{in only the training fold}, to reduce variance. The test folds are always left untrimmed/Winsorized so \cref{claim:1} remains valid. Explicitly we define Winsorization at level $0.001$ to Winsorize the $X, Y$ distributions at $P0.1$, $P99.9$ and the (positive) auxiliary $D$ distribution at $P99.9$.

% \subsubsection{Difference-of-Means (dm)}
The simple \textbf{difference-of-means estimator},
\begin{align}
	\hat{\Delta}_{DM}= \frac{1}{\abs{\cT}} \sum_{i \in \cT} Y_i(1) - \frac{1}{\abs{\cC}} \sum_{i \in \cC} Y_i(0), \label{eq:dm2}
\end{align} as defined before is the first estimator we consider.
%can be interpreted in a regression framework by writing $Y = Y(0)+T \cdot (Y(1)-Y(0))$. This implies we can estimate the ATE for the binary treatment using linear regression of the observed outcomes $Y_i$ on the vector $(1, T_i)$---which is equivalent to computing \cref{eq:dm2}.
% Under the assumption of randomization, taking expectations conditional on the treatment assignment yields:
% \begin{align}
	% \mE[Y | T] = \alpha + T \Delta \text{ where } \alpha = \mE[Y(0)].\label{eq:dm_cond}
	% \end{align}
%In this setting the noise model is heteroscedastic (and depends on $T$).
\label{subsec:dm}
We also consider the \textbf{Difference-of-Median-of-Means (mom) estimator}
%\subsubsection{Difference-of-Median-of-Means (mom)}
%Our definition of this estimator cannot be interpreted in the regression framework strictly speaking, but it is sufficiently similar that we describe it here. The formulation of \cref{eq:dm2} and relationship to \cref{eq:dm_cond} motivates the robust estimation of $\alpha$ and $\Delta$. %Equivalently, we replace the terms in $\frac{1}{\abs{\cT}} \sum_{i \in \cT} Y_i(1)$, $\frac{1}{\abs{\cC}} \sum_{i \in \cC} Y_i(0)$ with the median-of-means estimators for some prespecified block size $B$ to define,
\begin{align}
	\hat{\Delta}_{DMoM} = \MoM(\{ Y_{i}(1) \}_{i=1}^{\abs{\cT}}	, B) - \MoM(\{ Y_{i}(0) \}_{i=1}^{\abs{\cC}}		, B).
\end{align}
%Similarly, $\hat{\alpha} = \MoM(\{ Y_{i}(0) \}_{i=1}^{\abs{\cC}}		, B)$ to complete the regression analogy.
Where $\MoM(\{ Y_{i}(1) \}_{i=1}^{\abs{\cT}}	, B)$ indicates we bucket the data into $B$ blocks, compute the mean in each block, and the median across all the blocked means.
We use mom$1000$ in our experiments to denote the median-of-means estimator chosen with 1000 total blocks.
% \label{subsec:dmom} 
Next we also consider what we refer to as the \textbf{Generalized Difference-in-Differences (gen$\_$dd) estimator} which assumes access to a pretreatment item-specific covariate $X_i$ corresponding to the response value $Y_i$. So, assuming the model,
\begin{align}
	Y = \alpha + T \cdot \Delta + X \cdot \beta + \epsilon,
\end{align}
we can estimate the ATE for a binary treatment by (least-squares) regressing $Y_i$ onto $(1, T_i, X_i)$, where $\epsilon_i$ represents a general conditionally mean-zero noise term (which may depend on $X_i$). If the covariates $X_i$ are strongly correlated with the response value $Y_i$, incorporating them into the regression can significantly reduce the variance.
% \subsubsection{Generalized LR (and Generalized Difference-in-Differences) (gen$\_$dd)}
% \label{subsec:gen_dd}
% We are given access to a pretreatment item-specific covariate $X_i$ corresponding to the response value $Y_i$. If these covariates are strongly correlated with the response value $Y_i$, incorporating them into the regression can significantly reduce the variance. So, assuming the model,
% \begin{align}
	% 	Y = \alpha + T \cdot \Delta + X \cdot \beta + \epsilon,
	% \end{align}
%  we can estimate the ATE for a binary treatment by regressing $Y_i$ onto $(1, T_i, X_i)$, where $\epsilon_i$ represents a general conditionally mean-zero noise term (which may depend on $X_i$).

%  \begin{remark}
	% When the covariate $X$ is the pretreatment response variable we refer to the estimator as the \emph{generalized differences-of-differences estimator}, since the population moment equation can be written as $\mE[Y | X, T] = \alpha + T \Delta + X\beta$. The connection to the standard difference-of-differences estimator can be seen by forcing $\beta=1$ in the setting where $X$ is the pretreatment value of $Y$. Accordingly, an alternate interpretation of the difference-of-differences estimator is that it can be implemented by first regressing $Y_i-X_i$ onto $(1, T_i)$, which is equivalent to constructing,
	% \begin{align}
		% 	\hat{\Delta}_{DD}= \left(\frac{1}{\abs{\cT}} \sum_{i \in \cT} Y_{i}(1) - \frac{1}{\abs{\cT}} \sum_{i \in \cT} X_{i}(1) \right)- \left(\frac{1}{\abs{\cC}} \sum_{i \in \cC} Y_{i}(0) - \frac{1}{\abs{\cC}} \sum_{i \in \cC} X_{i}(0) \right). \label{eq:dd}
		% \end{align}
	% \end{remark}
% \label{subsec:gendd}
Finally we consider a reweighted version of the previous estimator we refer to as the \textbf{Weighted Generalized LR (and Generalized Difference-in-Differences) (gen$\_$dd$\_$w1)} estimator.
% \subsubsection{Weighted Generalized LR (and Generalized Difference-in-Differences) (gen$\_$dd$\_$w1)}
% \label{subsec:gen_dd_weight}
% Since all of the above estimators can be written as various forms of linear regression it is also possible to interpret them from the perspective of $M$-estimation as minimizing a sum of residuals defined as $e_i = Y_i-\alpha-\Delta T_i - X_i \beta$. 
That is, we can consider estimation objectives of the form:
% \begin{align}
	% 	\min_{\alpha, \Delta, \bm{\beta}} \sum_{i=1}^{n} \psi(e_i \cdot w_i),
	% \end{align}
% for some sequence of weights $w_i$. The choice we explore is that of simple weighted least-squares. That is, we take $\psi$ to be the squared loss and define the weights as $w = (1+D)^{-\gamma}$ (for $\gamma>0$) for some nonnegative covariate $D$. 
\begin{align}
	\frac{1}{n} \sum_{i=1}^n \frac{1}{(1+D_i)^\gamma} (Y_i - \alpha -\Delta T_i - \beta_i X_i)^2.
\end{align}
to estimate $\alpha$ $\beta$, and most importantly the TE $\Delta$. In practice, the covariate $D$ is taken as an auxiliary covariate, which serves as positive surrogate capturing the shape of the distribution of $Y$. In this case the weighting has the effect of downweighting large values of $Y$ which can be useful to regularize heavy-tailed distributions.
%By pushing the weighting function inside the loss we an alternative interpretation is that the prelab demand normalizes the response and feature vectors. That is we are effectively regressing $\frac{Y_i}{(1+D_i)^{\gamma/2}}$ onto $( \frac{1}{(1+D_i)^{\gamma/2}}, \frac{T_i}{(1+D_i)^{\gamma/2}}, \frac{X_i}{(1+D_i)^{\gamma/2}}$. Note that normalizing the ltfcf partially serves to stabilize the long-tail of the cash flow.

%In the first pass of our empirical analysis we compare several estimators as described in more detail above:
%\begin{itemize}
%	\item Difference-of-Means (dm): computed as exactly as previously described in \cref{subsec:dm} by differencing the mean post-treatment ltfcf between treatment and control.
%	\item Difference-of-Median-of-Means (mom): computed exactly as in \cref{subsec:dmom} by differencing the MoM of post-treatment ltfcf between treatment and control. The number of blocks was set arbitarily to 1000.
%	\item Generalized Difference-of-Differences (gen$\_$dd): computed exactly as in \cref{subsec:gen_dd} using the post-treatment ltfcf as $Y$, the pre-treatment ltfcf as $X$, and the treatment dummy as $T$.
%	\item Weighted Generalized Difference-of-Differences (gen$\_$dd$\_$wnum): computed exactly as in \cref{subsec:gen_dd_weight} using the post-treatment ltfcf as $Y$, the pre-treatment ltfcf as $X$, and the treatment dummy as $T$. The weights $w$ are computed using the pretreatment lab demand as $D$ and value $\gamma$ was varied between 1, 2, and 3, and for which the estimator is denoted gen$\_$dd$\_$w1, gen$\_$dd$\_$w2, gen$\_$dd$\_$w3 respectively.
%	\item Normalized Regression (gen$\_$dd$\_$w$\_$norm): computed exactly as in \cref{subsec:gen_dd_norm} using the post-treatment ltfcf as $Y$, the pre-treatment ltfcf as $X$, and the treatment dummy as $T$. The normalizations are computed using the pretreatment lab demand as $D$.
%	\item Polynomial Regressions in $X$ (gen$\_$dd$\_$polyltfcfnum): computed using the post-treatment ltfcf as $Y$, the pre-treatment ltfcf as $X$, and the treatment dummy as $T$ as in \cref{eq:polyltfcf}. The value num specifies the degree of the interaction.
%	\item Polylog Regressions in $D$ (gen$\_$dd$\_$polydemnum): computed using the post-treatment ltfcf as $Y$, the pre-treatment demand as $D$, and the treatment dummy as $T$ as in \cref{eq:polydemand}. The value num specifies the degree of the interaction\end{itemize}
%
%\cref{fig:error_across_labs_log} displays this phenomena quite explicitly for two different estimators.
%However, from \cref{fig:error_across_labs_90,,fig:error_across_labs_50} the error distribution of the weighted generalized difference-of-differences and winsorized difference-of-means estimator seems to generally be more left-skewed then that of the difference-in-means estimator--indicating the former are performing better then the latter. These insights are characteristic of our overall conclusions; we should be trading a large reduction in variance (via weighting or Winsorization) for a small increase in bias.

%\begin{figure}[!ht]
%\centering
%	\includegraphics[width=0.8\linewidth]{plots/hist_errs/error_hist_both_ests_log_xtrans_True_err_clip_100.pdf}
%	\caption{30-binned histogram of the number of labs vs log transformed cross-validated MSE (averaged over 100 resampled replicated) for the difference-of-means and the weighted generalized difference-of-differences estimators. The MSEs vary considerably over different labs and have large outliers.}
%	\label{fig:error_across_labs_log}
%\end{figure}
%
%\begin{figure}[!ht]
%\centering
%\begin{minipage}[b]{0.45\linewidth}
%	\centering
%	\includegraphics[width=0.8\linewidth]{plots_final_wins/hist_errs/error_hist_both_ests_log_xtrans_False_err_clip_90.pdf}
%	\caption{30-binned histogram of the number of labs vs their cross-validated Log MSE (averaged over 100 resampled replicates) for generalized differences-of-differences and the inverse demand weighted generalized difference-of-differences. Here the top $10\%$ of labs have been truncated. Inverse weighting decreases held-out errors.}
%	\label{fig:error_across_labs_90}
%\end{minipage}
%\quad
%\begin{minipage}[b]{0.45\linewidth}
%	\centering
%	\includegraphics[width=0.8\linewidth]{plots_final_wins/hist_errs/error_hist_both_ests_xtrans_False_err_clip_90.pdf}
%	\caption{30-binned histogram of the number of labs vs their cross-validated Log MSE (averaged over 100 resampled replicates) for difference-of-means and the winsorized difference-of-means estimators. Here the top $10\%$ of labs have been truncated. Winsorization reduces held-out-errors significantly.}
%	\label{fig:error_across_labs_50}
%\end{minipage}
%\end{figure}

%\subsection{An Aggregation Scheme}
%The above observations motivates the definition of a normalized score to compare the estimators $A$ vs $B$ which is a function of the vectors of their noisy errors\footnote{As noted before, in practice each error estimate is averaged over several resampled train/test splits but we suppress this extra notation for clarity.}:
%
%\begin{align}
%	\hat{\A} = \{ \MSE_{I_1, A}((\cT_1, \cC_1), (\cT_2, \cC_2)), \hdots, ...	 \MSE_{I_N, A}((\cT_1, \cC_1), (\cT_2, \cC_2)) \}
%\end{align}
%	vs
%\begin{align}
%	\hat{\B} =	\{ \MSE_{I_1, B}((\cT_1, \cC_1), (\cT_2, \cC_2)), \hdots, ...	, \MSE_{I_N, B}((\cT_1, \cC_1), (\cT_2, \cC_2)) \}
%\end{align}
%
%We define the normalized score vector of estimator $A$ vs $B$ as,
%\begin{align}
%	\score(\hat{\A}, \hat{\B}) =  \frac{\hat{\B}-\hat{\A}}{\hat{\A}+\hat{\B}}
%\end{align}
%where the division operator represents element-wise addition.
%This normalized score vector implicitly binarizes each of its elements to bound them in the range $[-1, 1]$. Each element of this vector is a noisy score of estimator $A$'s performance relative to $B$ \textit{on one lab in the corpus}\footnote{Our notion of a normalized score vector is element-wise transitive. That is $\frac{b-a}{a+b} > 0$ and $\frac{c-b}{b+c} > 0$ imply $\frac{c-a}{a+c}>0$.}. If the estimator has many elements that are positive, it suggests that estimator $B$ has larger errors than estimator $A$. In this case, we would expect estimator $A$ is better than estimator $B$.
%
%To mathematize this intuition we use the following heuristic which implicitly treats each lab equally independent of size. We use a two-sided one-sample $t$-test applied to this normalized score vector to test the null that the ``population mean" of the $\score$ ``distribution" is $0$: which corresponds to the case that the performance of estimator $A$ is indistinguishable from the performance of estimator $B$. Overall, this procedure interpolates between two extremes. A purely rank-based test of performance might only count the number of labs for which $A$ is better then $B$ irrespective of how much better one is in a particular AB test. While a procedure which only looks at the raw (unnormalized) lab errors has the property that labs with large MSE values for both estimators would drown out signal from labs with small MSE values. We stress that the $t$-test heuristic provides a simple way of converting the information contained in $\score(\hat{\A}, \hat{\B})$ to a single number, but we recommend looking at the score histograms for a more complete picture.
%
%Next we include histograms of the normalized score vectors for several estimators to aid intuition in our construction. In each histogram a left-skew indicates that in the score vector $\score(\hat{\A}, \hat{\B})$ estimator $A$ is performing better then estimator $B$. In \cref{fig:score_hist_dm_dm_wins,,fig:score_hist_dm_gen_dd,,fig:score_hist_dm_gen_dd_w1} we can see the difference-of-means estimator is dominated by both winsorized dm (dm$\_$wins.001), regression on the pretreatment ltfcf covariate (gen$\_$dd), and the inverse lab demand weighted generalized difference-of-differences estimator (gen$\_$dd$\_$w1). In \cref{fig:score_hist_gen_dd_dm_wins,,fig:score_hist_gen_dd_gen_dd_w1} we can see that the generalized difference-of-differences estimator (gen$\_$dd) is improved upon by winsorized differences-of-means (dm$\_$wins.001), and its reweighted version (gen$\_$dd$\_$w1) which both further reduce variance. Finally, directly comparing gen$\_$dd$\_$w1 vs dm$\_$wins.001 shows both estimators perform similarly; with the distribution having a long left tail but more mass in the mid-right then mid-left region. Finally, we can see in \cref{fig:score_hist_gen_dd_w1_gen_dd_w3} that both inverse weighting schemes (with powers varied) perform comparably. \cref{fig:score_hist_gen_dd_w1_gen_dd_w1_wins} seems to suggest combiningy Winsorization with inverse weighting/regression on the pretreatment covariate performs better then the latter two alone by more aggressively reducing variance. Finally, \cref{fig:score_hist_gen_dd_polyltfcf_gen_dd} shows that adding even second-order polynomial features in $X$ performs significantly worse then just gen$\_$dd alone. We found this to be universally true for all of the polynomial, polylog (in demand) regression methods and hence do not explore them further.


==> validation2.tex <==
%!TEX root = main.tex
\section{Results}
In this section we detail several simple and commonly used estimators for TE estimation and subsequently compare their relative performance.
\vspace{-0.2cm}

\subsection{Estimators}

For the following estimators, we note that each admits a ``Winsorization" which can be used to trade off bias and variance. To do this, we can simply Winsorize the covariates and targets, $X, D, Y$, \textit{in only the training fold}, to reduce variance. The test folds are always left untrimmed/Winsorized so \cref{claim:1} remains valid. Explicitly we define Winsorization at level $0.001$ to Winsorize the $X, Y$ distributions at $P0.1$, $P99.9$ and the (positive) auxiliary $D$ distribution at $P99.9$.

% \subsubsection{Difference-of-Means (dm)}
The simple \textbf{difference-of-means estimator},
\begin{align}
	\hat{\Delta}_{DM}= \frac{1}{\abs{\cT}} \sum_{i \in \cT} Y_i(1) - \frac{1}{\abs{\cC}} \sum_{i \in \cC} Y_i(0), \label{eq:dm2}
\end{align} as defined before is the first estimator we consider.
%can be interpreted in a regression framework by writing $Y = Y(0)+T \cdot (Y(1)-Y(0))$. This implies we can estimate the ATE for the binary treatment using linear regression of the observed outcomes $Y_i$ on the vector $(1, T_i)$---which is equivalent to computing \cref{eq:dm2}.
% Under the assumption of randomization, taking expectations conditional on the treatment assignment yields:
% \begin{align}
	% \mE[Y | T] = \alpha + T \Delta \text{ where } \alpha = \mE[Y(0)].\label{eq:dm_cond}
	% \end{align}
%In this setting the noise model is heteroscedastic (and depends on $T$).
\label{subsec:dm}
We also consider the \textbf{Difference-of-Median-of-Means (mom) estimator}
%\subsubsection{Difference-of-Median-of-Means (mom)}
%Our definition of this estimator cannot be interpreted in the regression framework strictly speaking, but it is sufficiently similar that we describe it here. The formulation of \cref{eq:dm2} and relationship to \cref{eq:dm_cond} motivates the robust estimation of $\alpha$ and $\Delta$. %Equivalently, we replace the terms in $\frac{1}{\abs{\cT}} \sum_{i \in \cT} Y_i(1)$, $\frac{1}{\abs{\cC}} \sum_{i \in \cC} Y_i(0)$ with the median-of-means estimators for some prespecified block size $B$ to define,
\begin{align}
	\hat{\Delta}_{DMoM} = \MoM(\{ Y_{i}(1) \}_{i=1}^{\abs{\cT}}	, B) - \MoM(\{ Y_{i}(0) \}_{i=1}^{\abs{\cC}}		, B).
\end{align}
%Similarly, $\hat{\alpha} = \MoM(\{ Y_{i}(0) \}_{i=1}^{\abs{\cC}}		, B)$ to complete the regression analogy.
Where $\MoM(\{ Y_{i}(1) \}_{i=1}^{\abs{\cT}}	, B)$ indicates we bucket the data into $B$ blocks, compute the mean in each block, and the median across all the blocked means.
We use mom$1000$ in our experiments to denote the median-of-means estimator chosen with 1000 total blocks.
% \label{subsec:dmom} 
Next we also consider what we refer to as the \textbf{Generalized Difference-in-Differences (gen$\_$dd) estimator} which assumes access to a pretreatment item-specific covariate $X_i$ corresponding to the response value $Y_i$. So, assuming the model,
\begin{align}
	Y = \alpha + T \cdot \Delta + X \cdot \beta + \epsilon,
\end{align}
we can estimate the ATE for a binary treatment by (least-squares) regressing $Y_i$ onto $(1, T_i, X_i)$, where $\epsilon_i$ represents a general conditionally mean-zero noise term (which may depend on $X_i$). If the covariates $X_i$ are strongly correlated with the response value $Y_i$, incorporating them into the regression can significantly reduce the variance.
% \subsubsection{Generalized LR (and Generalized Difference-in-Differences) (gen$\_$dd)}
% \label{subsec:gen_dd}
% We are given access to a pretreatment item-specific covariate $X_i$ corresponding to the response value $Y_i$. If these covariates are strongly correlated with the response value $Y_i$, incorporating them into the regression can significantly reduce the variance. So, assuming the model,
% \begin{align}
	% 	Y = \alpha + T \cdot \Delta + X \cdot \beta + \epsilon,
	% \end{align}
%  we can estimate the ATE for a binary treatment by regressing $Y_i$ onto $(1, T_i, X_i)$, where $\epsilon_i$ represents a general conditionally mean-zero noise term (which may depend on $X_i$).

%  \begin{remark}
	% When the covariate $X$ is the pretreatment response variable we refer to the estimator as the \emph{generalized differences-of-differences estimator}, since the population moment equation can be written as $\mE[Y | X, T] = \alpha + T \Delta + X\beta$. The connection to the standard difference-of-differences estimator can be seen by forcing $\beta=1$ in the setting where $X$ is the pretreatment value of $Y$. Accordingly, an alternate interpretation of the difference-of-differences estimator is that it can be implemented by first regressing $Y_i-X_i$ onto $(1, T_i)$, which is equivalent to constructing,
	% \begin{align}
		% 	\hat{\Delta}_{DD}= \left(\frac{1}{\abs{\cT}} \sum_{i \in \cT} Y_{i}(1) - \frac{1}{\abs{\cT}} \sum_{i \in \cT} X_{i}(1) \right)- \left(\frac{1}{\abs{\cC}} \sum_{i \in \cC} Y_{i}(0) - \frac{1}{\abs{\cC}} \sum_{i \in \cC} X_{i}(0) \right). \label{eq:dd}
		% \end{align}
	% \end{remark}
% \label{subsec:gendd}
Finally we consider a reweighted version of the previous estimator we refer to as the \textbf{Weighted Generalized LR (and Generalized Difference-in-Differences) (gen$\_$dd$\_$w1)} estimator.
% \subsubsection{Weighted Generalized LR (and Generalized Difference-in-Differences) (gen$\_$dd$\_$w1)}
% \label{subsec:gen_dd_weight}
% Since all of the above estimators can be written as various forms of linear regression it is also possible to interpret them from the perspective of $M$-estimation as minimizing a sum of residuals defined as $e_i = Y_i-\alpha-\Delta T_i - X_i \beta$. 
That is, we can consider estimation objectives of the form:
% \begin{align}
	% 	\min_{\alpha, \Delta, \bm{\beta}} \sum_{i=1}^{n} \psi(e_i \cdot w_i),
	% \end{align}
% for some sequence of weights $w_i$. The choice we explore is that of simple weighted least-squares. That is, we take $\psi$ to be the squared loss and define the weights as $w = (1+D)^{-\gamma}$ (for $\gamma>0$) for some nonnegative covariate $D$. 
\begin{align}
	\frac{1}{n} \sum_{i=1}^n \frac{1}{(1+D_i)^\gamma} (Y_i - \alpha -\Delta T_i - \beta_i X_i)^2.
\end{align}
to estimate $\alpha$ $\beta$, and most importantly the TE $\Delta$. In practice, the covariate $D$ is taken as an auxiliary covariate, which serves as positive surrogate capturing the shape of the distribution of $Y$. In this case the weighting has the effect of downweighting large values of $Y$ which can be useful to regularize heavy-tailed distributions.
%By pushing the weighting function inside the loss we an alternative interpretation is that the prelab demand normalizes the response and feature vectors. That is we are effectively regressing $\frac{Y_i}{(1+D_i)^{\gamma/2}}$ onto $( \frac{1}{(1+D_i)^{\gamma/2}}, \frac{T_i}{(1+D_i)^{\gamma/2}}, \frac{X_i}{(1+D_i)^{\gamma/2}}$. Note that normalizing the ltfcf partially serves to stabilize the long-tail of the cash flow.

%In the first pass of our empirical analysis we compare several estimators as described in more detail above:
%\begin{itemize}
%	\item Difference-of-Means (dm): computed as exactly as previously described in \cref{subsec:dm} by differencing the mean post-treatment ltfcf between treatment and control.
%	\item Difference-of-Median-of-Means (mom): computed exactly as in \cref{subsec:dmom} by differencing the MoM of post-treatment ltfcf between treatment and control. The number of blocks was set arbitarily to 1000.
%	\item Generalized Difference-of-Differences (gen$\_$dd): computed exactly as in \cref{subsec:gen_dd} using the post-treatment ltfcf as $Y$, the pre-treatment ltfcf as $X$, and the treatment dummy as $T$.
%	\item Weighted Generalized Difference-of-Differences (gen$\_$dd$\_$wnum): computed exactly as in \cref{subsec:gen_dd_weight} using the post-treatment ltfcf as $Y$, the pre-treatment ltfcf as $X$, and the treatment dummy as $T$. The weights $w$ are computed using the pretreatment lab demand as $D$ and value $\gamma$ was varied between 1, 2, and 3, and for which the estimator is denoted gen$\_$dd$\_$w1, gen$\_$dd$\_$w2, gen$\_$dd$\_$w3 respectively.
%	\item Normalized Regression (gen$\_$dd$\_$w$\_$norm): computed exactly as in \cref{subsec:gen_dd_norm} using the post-treatment ltfcf as $Y$, the pre-treatment ltfcf as $X$, and the treatment dummy as $T$. The normalizations are computed using the pretreatment lab demand as $D$.
%	\item Polynomial Regressions in $X$ (gen$\_$dd$\_$polyltfcfnum): computed using the post-treatment ltfcf as $Y$, the pre-treatment ltfcf as $X$, and the treatment dummy as $T$ as in \cref{eq:polyltfcf}. The value num specifies the degree of the interaction.
%	\item Polylog Regressions in $D$ (gen$\_$dd$\_$polydemnum): computed using the post-treatment ltfcf as $Y$, the pre-treatment demand as $D$, and the treatment dummy as $T$ as in \cref{eq:polydemand}. The value num specifies the degree of the interaction\end{itemize}
%
%\cref{fig:error_across_labs_log} displays this phenomena quite explicitly for two different estimators.
%However, from \cref{fig:error_across_labs_90,,fig:error_across_labs_50} the error distribution of the weighted generalized difference-of-differences and winsorized difference-of-means estimator seems to generally be more left-skewed then that of the difference-in-means estimator--indicating the former are performing better then the latter. These insights are characteristic of our overall conclusions; we should be trading a large reduction in variance (via weighting or Winsorization) for a small increase in bias.

%\begin{figure}[!ht]
%\centering
%	\includegraphics[width=0.8\linewidth]{plots/hist_errs/error_hist_both_ests_log_xtrans_True_err_clip_100.pdf}
%	\caption{30-binned histogram of the number of labs vs log transformed cross-validated MSE (averaged over 100 resampled replicated) for the difference-of-means and the weighted generalized difference-of-differences estimators. The MSEs vary considerably over different labs and have large outliers.}
%	\label{fig:error_across_labs_log}
%\end{figure}
%
%\begin{figure}[!ht]
%\centering
%\begin{minipage}[b]{0.45\linewidth}
%	\centering
%	\includegraphics[width=0.8\linewidth]{plots_final_wins/hist_errs/error_hist_both_ests_log_xtrans_False_err_clip_90.pdf}
%	\caption{30-binned histogram of the number of labs vs their cross-validated Log MSE (averaged over 100 resampled replicates) for generalized differences-of-differences and the inverse demand weighted generalized difference-of-differences. Here the top $10\%$ of labs have been truncated. Inverse weighting decreases held-out errors.}
%	\label{fig:error_across_labs_90}
%\end{minipage}
%\quad
%\begin{minipage}[b]{0.45\linewidth}
%	\centering
%	\includegraphics[width=0.8\linewidth]{plots_final_wins/hist_errs/error_hist_both_ests_xtrans_False_err_clip_90.pdf}
%	\caption{30-binned histogram of the number of labs vs their cross-validated Log MSE (averaged over 100 resampled replicates) for difference-of-means and the winsorized difference-of-means estimators. Here the top $10\%$ of labs have been truncated. Winsorization reduces held-out-errors significantly.}
%	\label{fig:error_across_labs_50}
%\end{minipage}
%\end{figure}

%\subsection{An Aggregation Scheme}
%The above observations motivates the definition of a normalized score to compare the estimators $A$ vs $B$ which is a function of the vectors of their noisy errors\footnote{As noted before, in practice each error estimate is averaged over several resampled train/test splits but we suppress this extra notation for clarity.}:
%
%\begin{align}
%	\hat{\A} = \{ \MSE_{I_1, A}((\cT_1, \cC_1), (\cT_2, \cC_2)), \hdots, ...	 \MSE_{I_N, A}((\cT_1, \cC_1), (\cT_2, \cC_2)) \}
%\end{align}
%	vs
%\begin{align}
%	\hat{\B} =	\{ \MSE_{I_1, B}((\cT_1, \cC_1), (\cT_2, \cC_2)), \hdots, ...	, \MSE_{I_N, B}((\cT_1, \cC_1), (\cT_2, \cC_2)) \}
%\end{align}
%
%We define the normalized score vector of estimator $A$ vs $B$ as,
%\begin{align}
%	\score(\hat{\A}, \hat{\B}) =  \frac{\hat{\B}-\hat{\A}}{\hat{\A}+\hat{\B}}
%\end{align}
%where the division operator represents element-wise addition.
%This normalized score vector implicitly binarizes each of its elements to bound them in the range $[-1, 1]$. Each element of this vector is a noisy score of estimator $A$'s performance relative to $B$ \textit{on one lab in the corpus}\footnote{Our notion of a normalized score vector is element-wise transitive. That is $\frac{b-a}{a+b} > 0$ and $\frac{c-b}{b+c} > 0$ imply $\frac{c-a}{a+c}>0$.}. If the estimator has many elements that are positive, it suggests that estimator $B$ has larger errors than estimator $A$. In this case, we would expect estimator $A$ is better than estimator $B$.
%
%To mathematize this intuition we use the following heuristic which implicitly treats each lab equally independent of size. We use a two-sided one-sample $t$-test applied to this normalized score vector to test the null that the ``population mean" of the $\score$ ``distribution" is $0$: which corresponds to the case that the performance of estimator $A$ is indistinguishable from the performance of estimator $B$. Overall, this procedure interpolates between two extremes. A purely rank-based test of performance might only count the number of labs for which $A$ is better then $B$ irrespective of how much better one is in a particular AB test. While a procedure which only looks at the raw (unnormalized) lab errors has the property that labs with large MSE values for both estimators would drown out signal from labs with small MSE values. We stress that the $t$-test heuristic provides a simple way of converting the information contained in $\score(\hat{\A}, \hat{\B})$ to a single number, but we recommend looking at the score histograms for a more complete picture.
%
%Next we include histograms of the normalized score vectors for several estimators to aid intuition in our construction. In each histogram a left-skew indicates that in the score vector $\score(\hat{\A}, \hat{\B})$ estimator $A$ is performing better then estimator $B$. In \cref{fig:score_hist_dm_dm_wins,,fig:score_hist_dm_gen_dd,,fig:score_hist_dm_gen_dd_w1} we can see the difference-of-means estimator is dominated by both winsorized dm (dm$\_$wins.001), regression on the pretreatment ltfcf covariate (gen$\_$dd), and the inverse lab demand weighted generalized difference-of-differences estimator (gen$\_$dd$\_$w1). In \cref{fig:score_hist_gen_dd_dm_wins,,fig:score_hist_gen_dd_gen_dd_w1} we can see that the generalized difference-of-differences estimator (gen$\_$dd) is improved upon by winsorized differences-of-means (dm$\_$wins.001), and its reweighted version (gen$\_$dd$\_$w1) which both further reduce variance. Finally, directly comparing gen$\_$dd$\_$w1 vs dm$\_$wins.001 shows both estimators perform similarly; with the distribution having a long left tail but more mass in the mid-right then mid-left region. Finally, we can see in \cref{fig:score_hist_gen_dd_w1_gen_dd_w3} that both inverse weighting schemes (with powers varied) perform comparably. \cref{fig:score_hist_gen_dd_w1_gen_dd_w1_wins} seems to suggest combiningy Winsorization with inverse weighting/regression on the pretreatment covariate performs better then the latter two alone by more aggressively reducing variance. Finally, \cref{fig:score_hist_gen_dd_polyltfcf_gen_dd} shows that adding even second-order polynomial features in $X$ performs significantly worse then just gen$\_$dd alone. We found this to be universally true for all of the polynomial, polylog (in demand) regression methods and hence do not explore them further.

\subsection{Estimator Comparisons}

In this section, we present results obtained from  a corpus of 699 RCTs performed at Amazon over several years as described in \cref{sec:data}. We compare estimators by their out-of-sample MSE computed via the cross-validation procedure described in \cref{sec:val}. 
%In our experiments, we resampled each treatment and control group into 50/50 splits over 100 different train/test replications. Our reported results for the mean-squared error (MSE) of a given estimator in a lab are averaged over all the held-out validation estimates of the MSE computed on these 100 train/test splits. [repetition]

We begin by studying several of the normalized score histograms to facilitate the comparison of our estimators; additional results are provided in \cref{app:additional}. In judging two estimators $A, B$ via their score distribution $\score(\hat{\A}, \hat{\B})$, we note that a left-skewed score distribution indicates $B$ is a better estimator (in terms of its MSE) than $A$.


\begin{figure}[!htb]
\minipage{0.32\textwidth}
\includegraphics[width=\linewidth]{Figures/score_hist_dm_vs_dm_wins001.pdf}
\caption{Histogram of the score distribution for dm vs Winsorized (at $0.001$) dm estimator.} \label{fig:score_hist_dm_dm_wins}
\endminipage\hfill
\minipage{0.32\textwidth}
\includegraphics[width=\linewidth]{Figures/score_hist_dm_vs_gen_dd.pdf}
\caption{Histogram of the score distribution for dm vs gen$\_$dd estimator.} \label{fig:score_hist_dm_gen_dd}
\endminipage\hfill
\minipage{0.32\textwidth}%
\includegraphics[width=\linewidth]{Figures/score_hist_dm_vs_gen_dd_w1.pdf}
\caption{Histogram of the score distribution for dm vs gen$\_$dd$\_$w1 estimator.} \label{fig:score_hist_dm_gen_dd_w1}
\endminipage
\end{figure}



%\begin{figure}[!ht]
%\centering
%\begin{minipage}[b]{0.3\linewidth}
%	\centering
%	\includegraphics[width=0.8\linewidth]{Figures/score_hist_dm_vs_dm_wins001.pdf}
%	\caption{Histogram of the score distribution for dm vs Winsorized (at $0.001$) dm estimator.}
%	\label{fig:score_hist_dm_dm_wins}
%\end{minipage}
%\quad
%\begin{minipage}[b]{0.3\linewidth}
%	\centering
%	\includegraphics[width=0.8\linewidth]{Figures/score_hist_dm_vs_gen_dd.pdf}
%	\caption{Histogram of the score distribution for dm vs gen$\_$dd estimator.}
%	\label{fig:score_hist_dm_gen_dd}
%\end{minipage}
%\quad
%\begin{minipage}[b]{0.3\linewidth}
%	\centering
%	\includegraphics[width=0.8\linewidth]{Figures/score_hist_dm_vs_gen_dd_w1.pdf}
%	\caption{Histogram of the score distribution for dm vs gen$\_$dd$\_$w1 estimator.}
%	\label{fig:score_hist_dm_gen_dd_w1}
%\end{minipage}
%\end{figure}

% \begin{figure}[!ht]
% \centering
% \begin{minipage}[b]{0.3\linewidth}
	% 	\centering
	% 	\includegraphics[width=0.8\linewidth]{plots_final_wins_fixed/hist_scores/score_hist_gen_dd_vs_dm_wins001.pdf}
	% 	\caption{Histogram of the score distribution for gen$\_$dd vs Winsorized (at $0.001$) dm estimator.}
	% \label{fig:score_hist_gen_dd_dm_wins}
	% \end{minipage}
% \quad
% \begin{minipage}[b]{0.3\linewidth}
	% 	\centering
	% 	\includegraphics[width=0.8\linewidth]{plots_final_wins_fixed/hist_scores/score_hist_gen_dd_vs_gen_dd_w1.pdf}
	% 	\caption{Histogram of the score distribution for gen$\_$dd vs gen$\_$dd$\_$w1 estimator.}
	% \label{fig:score_hist_gen_dd_gen_dd_w1}
	% \end{minipage}
% \quad
% \begin{minipage}[b]{0.3\linewidth}
	% 	\centering
	% 	\includegraphics[width=0.8\linewidth]{plots_final_wins_fixed/hist_scores/score_hist_gen_dd_w1_vs_dm_wins001.pdf}
	% 	\caption{Histogram of the score distribution for gen$\_$dd$\_$w1 vs Winsorized (at $0.001$) dm estimator.}
	% \label{fig:score_hist_gen_dd_w1_dm_wins}
	% \end{minipage}
% \end{figure}

% \begin{figure}[!ht]
% \centering
% \begin{minipage}[b]{0.3\linewidth}
	% 	\centering
	% 	\includegraphics[width=0.85\linewidth]{plots_final_wins_fixed/hist_scores/score_hist_gen_dd_w1_vs_gen_dd_w2.pdf}
	% 	\caption{Histogram of the score distribution for gen$\_$dd$\_$w1 vs gen$\_$dd$\_$w2 estimator.}
	% \label{fig:score_hist_gen_dd_w1_gen_dd_w3}
	% \end{minipage}
% \quad
% \begin{minipage}[b]{0.3\linewidth}
	% 	\centering
	% 	\includegraphics[width=0.85\linewidth]{plots_final_wins_fixed/hist_scores/score_hist_gen_dd_w1_vs_gen_dd_w1_wins001.pdf}
	% 	\caption{Histogram of the score distribution for gen$\_$dd$\_$w1 vs gen$\_$dd$\_$w1$\_$wins.001 estimator.}
	% 	\label{fig:score_hist_gen_dd_w1_gen_dd_w1_wins}
	% \end{minipage}
% \quad
% \begin{minipage}[b]{0.3\linewidth}
	% 	\centering
	% 	\includegraphics[width=0.85\linewidth]{plots_final_wins_fixed/hist_scores/score_hist_gen_dd_w3_vs_gen_dd_w1.pdf}
	% 	\caption{Histogram of the score distribution for gen$\_$dd$\_$w3 vs gen$\_$dd$\_$w1 estimator.}
	% 	\label{fig:score_hist_mom1000}
	% \end{minipage}
% \end{figure}



%Both, \cref{fig:score_hist_dm_gen_dd_weight,,fig:score_hist_dm_mom} are left-skewed indicating the dm estimator is dominated by gen$\_$dd$\_$weight and mom.
In \cref{tab:table0to100}, we use the $t$-test heuristic from \cref{sec:agg} to summarize each score histogram. For the sake of brevity, we do not display all the methods tested in the table.
%We found that all the estimators weighted by different powers ($1,2,3$) of the inverse $D$ distribution perform comparably. 
Overall, we see several phenomena that accord with our expectations. First, adjusting for the pretreatment covariate reduces variance (i.e., gen$\_$dd is better then dm). Second, downweighting large values of $Y$ provides significant value: inverse weighting by $D$ and Winsorization performs generically the best under our metric (gen$\_$dd$\_$w1 and all Winsorized estimators perform well). We also see that the dm estimator is dominated by every other method in \cref{tab:table0to100}; such as the median of median-of-means estimator (mom$1000$), whose robustness underlies its improved performance. 
%We can also check that the results from \cref{tab:table0to100} are stable with respect to different resampled replicates to compute the cross-validated errors which feed into the error vectors in $\hat{\A}$/$\hat{\B}$ as \cref{tab:tab1to50,,tab:tab51to100} in \cref{app:additional} show.

We summarize this table by converting it into a table of pairwise comparisons of wins/losses/ties using a $p$-value to determine the significance of the win or loss. The question of extracting an ordered ranking from the table of wins/losses is a classic problem. The natural procedure of simply summing up the number of row-wise wins is commonly referred to as the Copeland/Borda counting method (see \citep{saari1996copeland} and references within). 
%It has recently been shown that such a simple method is robust to the misspecification of the ranking model and optimal under minimal assumptions \citep{JMLR:v18:16-206}.\footnote{Such consistency results are not entirely necessary since our notion of a normalized score vector is element-wise transitive. That is, $\frac{b-a}{a+b} > 0$ and $\frac{c-b}{b+c} > 0$ imply $\frac{c-a}{a+c}>0$.}

\begin{table}[!htbp]
\caption{Comparison of Estimators via one-sample $t$-test applied to their normalized score vector. Easiest to read row-wise. The index $(A, B)$ of the table computes the pair of the ($t$-statistic, $p$-value) associated with the score $\score(\hat{\A}, \hat{\B})$. A large positive $t$-statistic at index $(A, B)$ indicates estimator $A$ is better then estimator $B$ and vice-versa.}
\label{tab:table0to100}
\centering
\resizebox{\columnwidth}{!}{%
	\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
		\hline
		Method &
		dm &
		mom1000 &
		gen\_dd &
		gen\_dd\_w1 &
		dm\_wins.001 &
		gen\_dd\_wins.001 &
		gen\_dd\_w1\_wins.001 \\ \hline
		dm &
		x &
		(-3.58, 0.000363) &
		(-12.68, 2.38e-33) &
		(-22.36, 3.6e-84) &
		(-28.19, 7.99e-118) &
		(-25.33, 2.96e-101) &
		(-24.96, 4.11e-99) \\ \hline
		mom1000 &
		(3.58, 0.000363) &
		x &
		(-2.12, 0.0342) &
		(-11.89, 7.32e-30) &
		(-13.51, 3.78e-37) &
		(-14.61, 1.94e-42) &
		(-15.72, 5.33e-48) \\ \hline
		gen\_dd &
		(12.68, 2.38e-33) &
		(2.12, 0.0342) &
		x &
		(-21.1, 4.73e-77) &
		(-19.01, 2e-65) &
		(-25.15, 3.11e-100) &
		(-23.49, 1.14e-90) \\ \hline
		gen\_dd\_w1 &
		(22.36, 3.6e-84) &
		(11.89, 7.32e-30) &
		(21.1, 4.73e-77) &
		x &
		(-0.26, 0.794) &
		(-5.12, 3.87e-07) &
		(-9.56, 1.87e-20) \\ \hline
		dm\_wins.001 &
		(28.19, 7.99e-118) &
		(13.51, 3.78e-37) &
		(19.01, 2e-65) &
		(0.26, 0.794) &
		x &
		(-4.17, 3.41e-05) &
		(-5.39, 9.62e-08) \\ \hline
		gen\_dd\_wins.001 &
		(25.33, 2.96e-101) &
		(14.61, 1.94e-42) &
		(25.15, 3.11e-100) &
		(5.12, 3.87e-07) &
		(4.17, 3.41e-05) &
		x &
		(-4.12, 4.2e-05) \\ \hline
		gen\_dd\_w1\_wins.001 & (24.96, 4.11e-99) & (15.72, 5.33e-48) & (23.49, 1.14e-90) & (9.56, 1.87e-20) & (5.39, 9.62e-08) & (4.12, 4.2e-05) & x \\ \hline
	\end{tabular}%
}
\end{table}


Applying such a method by inspection returns the following rankings:
\begin{align}
\textbf{gen$\_$dd$\_$w1$\_$wins.001} >
\textbf{gen$\_$dd$\_$wins.001} >
\textbf{dm$\_$wins.001} \approx
\textbf{gen$\_$dd$\_$w1} > \textbf{gen$\_$dd} > \textbf{mom1000} > \textbf{dm} \nonumber
\end{align}
Overall, these results suggest that aggressively Winsorizing and/or downweighting heavy tails can profitably trade variance for some additional bias. % We also stress that although our ranking procedure via $t$-statistics is transitive, the score and $t$-statistic values between $A$ and $B$ are computed via relative normalization between just these two estimator errors. Hence the actual values across several estimators are not always directly comparable due to the different normalizations used. Thus, we should always look at the performance of two estimators directly, take their score histogram into consideration, as well as exercise common-sense checks to draw further conclusions.

% the bias is always negative, right (if you remove largest outliers via winsorization)? what's the business cost of that, especially if the known risk of bias isn't communicated? 
